First results on ProtoDUNE-SP liquid argon time projection chamber performance from a beam test at the CERN Neutrino Platform

The ProtoDUNE-SP detector is a single-phase liquid argon time projection chamber with an active volume of $7.2\times 6.0\times 6.9$ m$^3$. It is installed at the CERN Neutrino Platform in a specially-constructed beam that delivers charged pions, kaons, protons, muons and electrons with momenta in the range 0.3 GeV$/c$ to 7 GeV/$c$. Beam line instrumentation provides accurate momentum measurements and particle identification. The ProtoDUNE-SP detector is a prototype for the first far detector module of the Deep Underground Neutrino Experiment, and it incorporates full-size components as designed for that module. This paper describes the beam line, the time projection chamber, the photon detectors, the cosmic-ray tagger, the signal processing and particle reconstruction. It presents the first results on ProtoDUNE-SP's performance, including noise and gain measurements, $dE/dx$ calibration for muons, protons, pions and electrons, drift electron lifetime measurements, and photon detector noise, signal sensitivity and time resolution measurements. The measured values meet or exceed the specifications for the DUNE far detector, in several cases by large margins. ProtoDUNE-SP's successful operation starting in 2018 and its production of large samples of high-quality data demonstrate the effectiveness of the single-phase far detector design.

==> alconvert/protoduneauthorlist-revtex.tex <==
%----------------------------------------------------
% List of institutions, need not be alphabetical
% Need to also add institution as \affiliation below this to get alphabetical order right
\newcommand{\Amsterdam}{University of Amsterdam, NL-1098 XG Amsterdam, The Netherlands}
\newcommand{\Antananarivo}{University of Antananarivo, Antananarivo 101, Madagascar}
\newcommand{\AntonioNarino}{Universidad Antonio Nari{\~n}o, Bogot{\'a}, Colombia}
\newcommand{\Argonne}{Argonne National Laboratory, Argonne, IL 60439, USA}
\newcommand{\Arizona}{University of Arizona, Tucson, AZ 85721, USA}
\newcommand{\Asuncion}{Universidad Nacional de Asunci{\'o}n, San Lorenzo, Paraguay}
\newcommand{\Athens}{University of Athens, Zografou GR 157 84, Greece}
\newcommand{\Atlantico}{Universidad del Atl{\'a}ntico, Atl{\'a}ntico, Colombia}
\newcommand{\Banaras}{Banaras Hindu University, Varanasi - 221 005, India}
\newcommand{\Basel}{University of Basel, CH-4056 Basel, Switzerland}
\newcommand{\Bern}{University of Bern, CH-3012 Bern, Switzerland}
\newcommand{\Beykent}{Beykent University, Istanbul, Turkey}
\newcommand{\Birmingham}{University of Birmingham, Birmingham B15 2TT, United Kingdom}
\newcommand{\BolognaUniversity}{Universit{\`a} del Bologna, 40127 Bologna, Italy}
\newcommand{\Boston}{Boston University, Boston, MA 02215, USA}
\newcommand{\Bristol}{University of Bristol, Bristol BS8 1TL, United Kingdom}
\newcommand{\Brookhaven}{Brookhaven National Laboratory, Upton, NY 11973, USA}
\newcommand{\Bucharest}{University of Bucharest, Bucharest, Romania}
\newcommand{\CBPF}{Centro Brasileiro de Pesquisas F\'isicas, Rio de Janeiro, RJ 22290-180, Brazil}
\newcommand{\CEASaclay}{CEA/Saclay, IRFU Institut de Recherche sur les Lois Fondamentales de l'Univers, F-91191 Gif-sur-Yvette CEDEX, France}
\newcommand{\CERN}{CERN, The European Organization for Nuclear Research, 1211 Meyrin, Switzerland}
\newcommand{\CIEMAT}{CIEMAT, Centro de Investigaciones Energ{\'e}ticas, Medioambientales y Tecnol{\'o}gicas, E-28040 Madrid, Spain}
\newcommand{\CUSB}{Central University of South Bihar, Gaya {\textendash} 824236, India }
\newcommand{\CalBerkeley}{University of California Berkeley, Berkeley, CA 94720, USA}
\newcommand{\CalDavis}{University of California Davis, Davis, CA 95616, USA}
\newcommand{\CalIrvine}{University of California Irvine, Irvine, CA 92697, USA}
\newcommand{\CalLosangeles}{University of California Los Angeles, Los Angeles, CA 90095, USA}
\newcommand{\CalRiverside}{University of California Riverside, Riverside CA 92521, USA}
\newcommand{\CalSantabarbara}{University of California Santa Barbara, Santa Barbara, California 93106 USA}
\newcommand{\Caltech}{California Institute of Technology, Pasadena, CA 91125, USA}
\newcommand{\Cambridge}{University of Cambridge, Cambridge CB3 0HE, United Kingdom}
\newcommand{\Campinas}{Universidade Estadual de Campinas, Campinas - SP, 13083-970, Brazil}
\newcommand{\CataniaUniversitadi}{Universit{\`a} di Catania, 2 - 95131 Catania, Italy}
\newcommand{\Charles}{Institute of Particle and Nuclear Physics of the Faculty of Mathematics and Physics of the Charles University, 180 00 Prague 8, Czech Republic }
\newcommand{\Chicago}{University of Chicago, Chicago, IL 60637, USA}
\newcommand{\ChungAng}{Chung-Ang University, Seoul 06974, South Korea}
\newcommand{\Cincinnati}{University of Cincinnati, Cincinnati, OH 45221, USA}
\newcommand{\Cinvestav}{Centro de Investigaci{\'o}n y de Estudios Avanzados del Instituto Polit{\'e}cnico Nacional (Cinvestav), Mexico City, Mexico}
\newcommand{\Colima}{Universidad de Colima, Colima, Mexico}
\newcommand{\ColoradoBoulder}{University of Colorado Boulder, Boulder, CO 80309, USA}
\newcommand{\ColoradoState}{Colorado State University, Fort Collins, CO 80523, USA}
\newcommand{\Columbia}{Columbia University, New York, NY 10027, USA}
\newcommand{\CzechAcademyofSciences}{Institute of Physics, Czech Academy of Sciences, 182 00 Prague 8, Czech Republic}
\newcommand{\CzechTechnical}{Czech Technical University, 115 19 Prague 1, Czech Republic}
\newcommand{\DakotaState}{Dakota State University, Madison, SD 57042, USA}
\newcommand{\Dallas}{University of Dallas, Irving, TX 75062-4736, USA}
\newcommand{\DannecyleVieux}{Laboratoire d'Annecy-le-Vieux de Physique des Particules, CNRS/IN2P3 and Universit{\'e} Savoie Mont Blanc, 74941 Annecy-le-Vieux, France}
\newcommand{\Daresbury}{Daresbury Laboratory, Cheshire WA4 4AD, United Kingdom}
\newcommand{\Drexel}{Drexel University, Philadelphia, PA 19104, USA}
\newcommand{\Duke}{Duke University, Durham, NC 27708, USA}
\newcommand{\Durham}{Durham University, Durham DH1 3LE, United Kingdom}
\newcommand{\EIA}{Universidad EIA, Antioquia, Colombia}
\newcommand{\ETH}{ETH Zurich, Zurich, Switzerland}
\newcommand{\Edinburgh}{University of Edinburgh, Edinburgh EH8 9YL, United Kingdom}
\newcommand{\FCULport}{Faculdade de Ci{\^e}ncias da Universidade de Lisboa - FCUL, 1749-016 Lisboa, Portugal}
\newcommand{\FederaldeAlfenas}{Universidade Federal de Alfenas, Po{\c{c}}os de Caldas - MG, 37715-400, Brazil}
\newcommand{\FederaldeGoias}{Universidade Federal de Goias, Goiania, GO 74690-900, Brazil}
\newcommand{\FederaldeSaoCarlos}{Universidade Federal de S{\~a}o Carlos, Araras - SP, 13604-900, Brazil}
\newcommand{\FederaldoABC}{Universidade Federal do ABC, Santo Andr{\'e} - SP, 09210-580 Brazil}
\newcommand{\FederaldoRio}{Universidade Federal do Rio de Janeiro,  Rio de Janeiro - RJ, 21941-901, Brazil}
\newcommand{\Fermi}{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\newcommand{\Florida}{University of Florida, Gainesville, FL 32611-8440, USA}
\newcommand{\Fluminense}{Fluminense Federal University, 9 Icara{\'\i} Niter{\'o}i - RJ, 24220-900, Brazil }
\newcommand{\Genova}{Universit{\`a} degli Studi di Genova, Genova, Italy}
\newcommand{\Georgian}{Georgian Technical University, Tbilisi, Georgia}
\newcommand{\GranSasso}{Gran Sasso Science Institute, L'Aquila, Italy}
\newcommand{\GranSassoLab}{Laboratori Nazionali del Gran Sasso, L'Aquila AQ, Italy}
\newcommand{\Granada}{University of Granada {\&} CAFPE, 18002 Granada, Spain}
\newcommand{\Grenoble}{University Grenoble Alpes, CNRS, Grenoble INP, LPSC-IN2P3, 38000 Grenoble, France}
\newcommand{\Guanajuato}{Universidad de Guanajuato, Guanajuato, C.P. 37000, Mexico}
\newcommand{\Harish}{Harish-Chandra Research Institute, Jhunsi, Allahabad 211 019, India}
\newcommand{\Harvard}{Harvard University, Cambridge, MA 02138, USA}
\newcommand{\Hawaii}{University of Hawaii, Honolulu, HI 96822, USA}
\newcommand{\Houston}{University of Houston, Houston, TX 77204, USA}
\newcommand{\Hyderabad}{University of  Hyderabad, Gachibowli, Hyderabad - 500 046, India}
\newcommand{\IFAE}{Institut de F{\`\i}sica d'Altes Energies, Barcelona, Spain}
\newcommand{\IFIC}{Instituto de Fisica Corpuscular, 46980 Paterna, Valencia, Spain}
\newcommand{\IHEP}{Institute of High Energy Physics, 100049 Beijing, China}
\newcommand{\INFNBologna}{Istituto Nazionale di Fisica Nucleare Sezione di Bologna, 40127 Bologna BO, Italy}
\newcommand{\INFNCatania}{Istituto Nazionale di Fisica Nucleare Sezione di Catania, I-95123 Catania, Italy}
\newcommand{\INFNGenova}{Istituto Nazionale di Fisica Nucleare Sezione di Genova, 16146 Genova GE, Italy}
\newcommand{\INFNLecce}{Istituto Nazionale di Fisica Nucleare Sezione di Lecce, 73100 - Lecce, Italy}
\newcommand{\INFNMilanBicocca}{Istituto Nazionale di Fisica Nucleare Sezione di Milano Bicocca, 3 - I-20126 Milano, Italy}
\newcommand{\INFNMilano}{Istituto Nazionale di Fisica Nucleare Sezione di Milano, 20133 Milano, Italy}
\newcommand{\INFNNapoli}{Istituto Nazionale di Fisica Nucleare Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\INFNPadova}{Istituto Nazionale di Fisica Nucleare Sezione di Padova, 35131 Padova, Italy}
\newcommand{\INFNPavia}{Istituto Nazionale di Fisica Nucleare Sezione di Pavia,  I-27100 Pavia, Italy}
\newcommand{\INFNSud}{Istituto Nazionale di Fisica Nucleare Laboratori Nazionali del Sud, 95123 Catania, Italy}
\newcommand{\INR}{Institute for Nuclear Research of the Russian Academy of Sciences, Moscow 117312, Russia}
\newcommand{\IPLyon}{Institut de Physique des 2 Infinis de Lyon, 69622 Villeurbanne, France}
\newcommand{\IPM}{Institute for Research in Fundamental Sciences, Tehran, Iran}
\newcommand{\ISTlisboa}{Instituto Superior T{\'e}cnico - IST, Universidade de Lisboa, Portugal}
\newcommand{\Idaho}{Idaho State University, Pocatello, ID 83209, USA}
\newcommand{\Illinoisinstitute}{Illinois Institute of Technology, Chicago, IL 60616, USA}
\newcommand{\Imperial}{Imperial College of Science Technology and Medicine, London SW7 2BZ, United Kingdom}
\newcommand{\IndGuwahati}{Indian Institute of Technology Guwahati, Guwahati, 781 039, India}
\newcommand{\IndHyderabad}{Indian Institute of Technology Hyderabad, Hyderabad, 502285, India}
\newcommand{\Indiana}{Indiana University, Bloomington, IN 47405, USA}
\newcommand{\Ingenieria}{Universidad Nacional de Ingenier{\'\i}a, Lima 25, Per{\'u}}
\newcommand{\Iowa}{University of Iowa, Iowa City, IA 52242, USA}
\newcommand{\IowaState}{Iowa State University, Ames, Iowa 50011, USA}
\newcommand{\Iwate}{Iwate University, Morioka, Iwate 020-8551, Japan}
\newcommand{\Jammu}{University of Jammu, Jammu-180006, India}
\newcommand{\Jawaharlal}{Jawaharlal Nehru University, New Delhi 110067, India}
\newcommand{\Jeonbuk}{Jeonbuk National University, Jeonrabuk-do 54896, South Korea}
\newcommand{\Jyvaskyla}{University of Jyvaskyla, FI-40014, Finland}
\newcommand{\KEK}{High Energy Accelerator Research Organization (KEK), Ibaraki, 305-0801, Japan}
\newcommand{\KISTI}{Korea Institute of Science and Technology Information, Daejeon, 34141, South Korea}
\newcommand{\KL}{K L University, Vaddeswaram, Andhra Pradesh 522502, India}
\newcommand{\Kansasstate}{Kansas State University, Manhattan, KS 66506, USA}
\newcommand{\Kavli}{Kavli Institute for the Physics and Mathematics of the Universe, Kashiwa, Chiba 277-8583, Japan}
\newcommand{\Kure}{National Institute of Technology, Kure College, Hiroshima, 737-8506, Japan}
\newcommand{\Kyiv}{Kyiv National University, 01601 Kyiv, Ukraine}
\newcommand{\LIP}{Laborat{\'o}rio de Instrumenta{\c{c}}{\~a}o e F{\'\i}sica Experimental de Part{\'\i}culas, 1649-003 Lisboa and 3004-516 Coimbra, Portugal}
\newcommand{\Lal}{Laboratoire de l'Acc{\'e}l{\'e}rateur Lin{\'e}aire, 91440 Orsay, France}
\newcommand{\Lancaster}{Lancaster University, Lancaster LA1 4YB, United Kingdom}
\newcommand{\LawrenceBerkeley}{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\newcommand{\Liverpool}{University of Liverpool, L69 7ZE, Liverpool, United Kingdom}
\newcommand{\LosAlmos}{Los Alamos National Laboratory, Los Alamos, NM 87545, USA}
\newcommand{\Louisanastate}{Louisiana State University, Baton Rouge, LA 70803, USA}
\newcommand{\Lucknow}{University of Lucknow, Uttar Pradesh 226007, India}
\newcommand{\Madrid}{Madrid Autonoma University and IFT UAM/CSIC, 28049 Madrid, Spain}
\newcommand{\Manchester}{University of Manchester, Manchester M13 9PL, United Kingdom}
\newcommand{\Massinsttech}{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
\newcommand{\Michigan}{University of Michigan, Ann Arbor, MI 48109, USA}
\newcommand{\Michiganstate}{Michigan State University, East Lansing, MI 48824, USA}
\newcommand{\MilanoBicocca}{Universit{\`a} del Milano-Bicocca, 20126 Milano, Italy}
\newcommand{\MilanoUniv}{Universit{\`a} degli Studi di Milano, I-20133 Milano, Italy}
\newcommand{\Minnduluth}{University of Minnesota Duluth, Duluth, MN 55812, USA}
\newcommand{\Minntwin}{University of Minnesota Twin Cities, Minneapolis, MN 55455, USA}
\newcommand{\Mississippi}{University of Mississippi, University, MS 38677 USA}
\newcommand{\NCNR}{National Centre for Nuclear Research, A. Soltana 7, 05 400 Otwock, Poland}
\newcommand{\Newmexico}{University of New Mexico, Albuquerque, NM 87131, USA}
\newcommand{\Niewodniczanski}{H. Niewodnicza{\'n}ski Institute of Nuclear Physics, Polish Academy of Sciences, Cracow, Poland}
\newcommand{\Nikhef}{Nikhef National Institute of Subatomic Physics, 1098 XG Amsterdam, Netherlands}
\newcommand{\Northdakota}{University of North Dakota, Grand Forks, ND 58202-8357, USA}
\newcommand{\Northernillinois}{Northern Illinois University, DeKalb, Illinois 60115, USA}
\newcommand{\Northwestern}{Northwestern University, Evanston, Il 60208, USA}
\newcommand{\NotreDame}{University of Notre Dame, Notre Dame, IN 46556, USA}
\newcommand{\Ohiostate}{Ohio State University, Columbus, OH 43210, USA}
\newcommand{\OregonState}{Oregon State University, Corvallis, OR 97331, USA}
\newcommand{\Oxford}{University of Oxford, Oxford, OX1 3RH, United Kingdom}
\newcommand{\PacificNorthwest}{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\newcommand{\Padova}{Universt{\`a} degli Studi di Padova, I-35131 Padova, Italy}
\newcommand{\Parisuniversite}{Universit{\'e} de Paris, CNRS, Astroparticule et Cosmologie, F-75006, Paris, France}
\newcommand{\Pavia}{Universit{\`a} degli Studi di Pavia, 27100 Pavia PV, Italy}
\newcommand{\Penn}{University of Pennsylvania, Philadelphia, PA 19104, USA}
\newcommand{\PennState}{Pennsylvania State University, University Park, PA 16802, USA}
\newcommand{\PhysicalResearchLaboratory}{Physical Research Laboratory, Ahmedabad 380 009, India}
\newcommand{\Pisa}{Universit{\`a} di Pisa, I-56127 Pisa, Italy}
\newcommand{\Pitt}{University of Pittsburgh, Pittsburgh, PA 15260, USA}
\newcommand{\Pontificia}{Pontificia Universidad Cat{\'o}lica del Per{\'u}, Lima, Per{\'u}}
\newcommand{\PuertoRico}{University of Puerto Rico, Mayaguez 00681, Puerto Rico, USA}
\newcommand{\Punjab}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\Radboud}{Radboud University, NL-6525 AJ Nijmegen, Netherlands}
\newcommand{\Rochester}{University of Rochester, Rochester, NY 14627, USA}
\newcommand{\Royalholloway}{Royal Holloway College London, TW20 0EX, United Kingdom}
\newcommand{\Rutgers}{Rutgers University, Piscataway, NJ, 08854, USA}
\newcommand{\Rutherford}{STFC Rutherford Appleton Laboratory, Didcot OX11 0QX, United Kingdom}
\newcommand{\SLAC}{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\newcommand{\SURF}{Sanford Underground Research Facility, Lead, SD, 57754, USA}
\newcommand{\Salento}{Universit{\`a} del Salento, 73100 Lecce, Italy}
\newcommand{\SergioArboleda}{Universidad Sergio Arboleda, 11022 Bogot{\'a}, Colombia}
\newcommand{\Sheffield}{University of Sheffield, Sheffield S3 7RH, United Kingdom}
\newcommand{\SouthDakotaSchool}{South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\newcommand{\SouthDakotaState}{South Dakota State University, Brookings, SD 57007, USA}
\newcommand{\Southcarolina}{University of South Carolina, Columbia, SC 29208, USA}
\newcommand{\SouthernMethodist}{Southern Methodist University, Dallas, TX 75275, USA}
\newcommand{\StonyBrook}{Stony Brook University, SUNY, Stony Brook, New York 11794, USA}
\newcommand{\SunYatSen}{Sun Yat-Sen University, 510275 Guangzhou, China}
\newcommand{\Sussex}{University of Sussex, Brighton, BN1 9RH, United Kingdom}
\newcommand{\Syracuse}{Syracuse University, Syracuse, NY 13244, USA}
\newcommand{\Tennknox}{University of Tennessee at Knoxville, TN, 37996, USA}
\newcommand{\TexasAM}{Texas A{\&}M University - Corpus Christi, Corpus Christi, TX 78412, USA}
\newcommand{\TexasArlington}{University of Texas at Arlington, Arlington, TX 76019, USA}
\newcommand{\Texasaustin}{University of Texas at Austin, Austin, TX 78712, USA}
\newcommand{\Toronto}{University of Toronto, Toronto, Ontario M5S 1A1, Canada}
\newcommand{\Tufts}{Tufts University, Medford, MA 02155, USA}
\newcommand{\Unifesp}{Universidade Federal de S{\~a}o Paulo, 09913-030, S{\~a}o Paulo, Brazil}
\newcommand{\UniversityCollegeLondon}{University College London, London, WC1E 6BT, United Kingdom}
\newcommand{\ValleyCity}{Valley City State University, Valley City, ND 58072, USA}
\newcommand{\VariableEnergy}{Variable Energy Cyclotron Centre, 700 064 West Bengal, India}
\newcommand{\VirginiaTech}{Virginia Tech, Blacksburg, VA 24060, USA}
\newcommand{\Warsaw}{University of Warsaw, 00-927 Warsaw, Poland}
\newcommand{\Warwick}{University of Warwick, Coventry CV4 7AL, United Kingdom}
\newcommand{\Wichita}{Wichita State University, Wichita, KS 67260, USA}
\newcommand{\WilliamMary}{William and Mary, Williamsburg, VA 23187, USA}
\newcommand{\Wisconsin}{University of Wisconsin Madison, Madison, WI 53706, USA}
\newcommand{\Yale}{Yale University, New Haven, CT 06520, USA}
\newcommand{\Yerevan}{Yerevan Institute for Theoretical Physics and Modeling, Yerevan 0036, Armenia}
\newcommand{\York}{York University, Toronto M3J 1P3, Canada}
%----------------------------------------------------
% So that institutions appear in alphabetical order:
\affiliation{\Amsterdam}
\affiliation{\Antananarivo}
\affiliation{\AntonioNarino}
\affiliation{\Argonne}
\affiliation{\Arizona}
\affiliation{\Asuncion}
\affiliation{\Athens}
\affiliation{\Atlantico}
\affiliation{\Banaras}
\affiliation{\Basel}
\affiliation{\Bern}
\affiliation{\Beykent}
\affiliation{\Birmingham}
\affiliation{\BolognaUniversity}
\affiliation{\Boston}
\affiliation{\Bristol}
\affiliation{\Brookhaven}
\affiliation{\Bucharest}
\affiliation{\CBPF}
\affiliation{\CEASaclay}
\affiliation{\CERN}
\affiliation{\CIEMAT}
\affiliation{\CUSB}
\affiliation{\CalBerkeley}
\affiliation{\CalDavis}
\affiliation{\CalIrvine}
\affiliation{\CalLosangeles}
\affiliation{\CalRiverside}
\affiliation{\CalSantabarbara}
\affiliation{\Caltech}
\affiliation{\Cambridge}
\affiliation{\Campinas}
\affiliation{\CataniaUniversitadi}
\affiliation{\Charles}
\affiliation{\Chicago}
\affiliation{\ChungAng}
\affiliation{\Cincinnati}
\affiliation{\Cinvestav}
\affiliation{\Colima}
\affiliation{\ColoradoBoulder}
\affiliation{\ColoradoState}
\affiliation{\Columbia}
\affiliation{\CzechAcademyofSciences}
\affiliation{\CzechTechnical}
\affiliation{\DakotaState}
\affiliation{\Dallas}
\affiliation{\DannecyleVieux}
\affiliation{\Daresbury}
\affiliation{\Drexel}
\affiliation{\Duke}
\affiliation{\Durham}
\affiliation{\EIA}
\affiliation{\ETH}
\affiliation{\Edinburgh}
\affiliation{\FCULport}
\affiliation{\FederaldeAlfenas}
\affiliation{\FederaldeGoias}
\affiliation{\FederaldeSaoCarlos}
\affiliation{\FederaldoABC}
\affiliation{\FederaldoRio}
\affiliation{\Fermi}
\affiliation{\Florida}
\affiliation{\Fluminense}
\affiliation{\Genova}
\affiliation{\Georgian}
\affiliation{\GranSasso}
\affiliation{\GranSassoLab}
\affiliation{\Granada}
\affiliation{\Grenoble}
\affiliation{\Guanajuato}
\affiliation{\Harish}
\affiliation{\Harvard}
\affiliation{\Hawaii}
\affiliation{\Houston}
\affiliation{\Hyderabad}
\affiliation{\IFAE}
\affiliation{\IFIC}
\affiliation{\IHEP}
\affiliation{\INFNBologna}
\affiliation{\INFNCatania}
\affiliation{\INFNGenova}
\affiliation{\INFNLecce}
\affiliation{\INFNMilanBicocca}
\affiliation{\INFNMilano}
\affiliation{\INFNNapoli}
\affiliation{\INFNPadova}
\affiliation{\INFNPavia}
\affiliation{\INFNSud}
\affiliation{\INR}
\affiliation{\IPLyon}
\affiliation{\IPM}
\affiliation{\ISTlisboa}
\affiliation{\Idaho}
\affiliation{\Illinoisinstitute}
\affiliation{\Imperial}
\affiliation{\IndGuwahati}
\affiliation{\IndHyderabad}
\affiliation{\Indiana}
\affiliation{\Ingenieria}
\affiliation{\Iowa}
\affiliation{\IowaState}
\affiliation{\Iwate}
\affiliation{\Jammu}
\affiliation{\Jawaharlal}
\affiliation{\Jeonbuk}
\affiliation{\Jyvaskyla}
\affiliation{\KEK}
\affiliation{\KISTI}
\affiliation{\KL}
\affiliation{\Kansasstate}
\affiliation{\Kavli}
\affiliation{\Kure}
\affiliation{\Kyiv}
\affiliation{\LIP}
\affiliation{\Lal}
\affiliation{\Lancaster}
\affiliation{\LawrenceBerkeley}
\affiliation{\Liverpool}
\affiliation{\LosAlmos}
\affiliation{\Louisanastate}
\affiliation{\Lucknow}
\affiliation{\Madrid}
\affiliation{\Manchester}
\affiliation{\Massinsttech}
\affiliation{\Michigan}
\affiliation{\Michiganstate}
\affiliation{\MilanoBicocca}
\affiliation{\MilanoUniv}
\affiliation{\Minnduluth}
\affiliation{\Minntwin}
\affiliation{\Mississippi}
\affiliation{\NCNR}
\affiliation{\Newmexico}
\affiliation{\Niewodniczanski}
\affiliation{\Nikhef}
\affiliation{\Northdakota}
\affiliation{\Northernillinois}
\affiliation{\Northwestern}
\affiliation{\NotreDame}
\affiliation{\Ohiostate}
\affiliation{\OregonState}
\affiliation{\Oxford}
\affiliation{\PacificNorthwest}
\affiliation{\Padova}
\affiliation{\Parisuniversite}
\affiliation{\Pavia}
\affiliation{\Penn}
\affiliation{\PennState}
\affiliation{\PhysicalResearchLaboratory}
\affiliation{\Pisa}
\affiliation{\Pitt}
\affiliation{\Pontificia}
\affiliation{\PuertoRico}
\affiliation{\Punjab}
\affiliation{\Radboud}
\affiliation{\Rochester}
\affiliation{\Royalholloway}
\affiliation{\Rutgers}
\affiliation{\Rutherford}
\affiliation{\SLAC}
\affiliation{\SURF}
\affiliation{\Salento}
\affiliation{\SergioArboleda}
\affiliation{\Sheffield}
\affiliation{\SouthDakotaSchool}
\affiliation{\SouthDakotaState}
\affiliation{\Southcarolina}
\affiliation{\SouthernMethodist}
\affiliation{\StonyBrook}
\affiliation{\SunYatSen}
\affiliation{\Sussex}
\affiliation{\Syracuse}
\affiliation{\Tennknox}
\affiliation{\TexasAM}
\affiliation{\TexasArlington}
\affiliation{\Texasaustin}
\affiliation{\Toronto}
\affiliation{\Tufts}
\affiliation{\Unifesp}
\affiliation{\UniversityCollegeLondon}
\affiliation{\ValleyCity}
\affiliation{\VariableEnergy}
\affiliation{\VirginiaTech}
\affiliation{\Warsaw}
\affiliation{\Warwick}
\affiliation{\Wichita}
\affiliation{\WilliamMary}
\affiliation{\Wisconsin}
\affiliation{\Yale}
\affiliation{\Yerevan}
\affiliation{\York}
%----------------------------------------------------
% Authors in alphabetical order
\author{B.~Abi} \affiliation{\Oxford}
\author{A.~Abed Abud} \affiliation{\CERN}\affiliation{\Liverpool}
\author{R.~Acciarri} \affiliation{\Fermi}
\author{M.~A.~Acero} \affiliation{\Atlantico}
\author{G.~Adamov} \affiliation{\Georgian}
\author{M.~Adamowski} \affiliation{\Fermi}
\author{D.~Adams} \affiliation{\Brookhaven}
\author{P.~Adrien} \affiliation{\CERN}
\author{M.~Adinolfi} \affiliation{\Bristol}
\author{Z.~Ahmad} \affiliation{\VariableEnergy}
\author{J.~Ahmed} \affiliation{\Warwick}
\author{T.~Alion} \affiliation{\Sussex}
\author{S.~Alonso Monsalve} \affiliation{\CERN}
\author{C.~Alt} \affiliation{\ETH}
\author{J.~Anderson} \affiliation{\Argonne}
\author{C.~Andreopoulos} \affiliation{\Rutherford}\affiliation{\Liverpool}
\author{M.~P.~Andrews} \affiliation{\Fermi}
\author{F.~Andrianala} \affiliation{\Antananarivo}
\author{S.~Andringa} \affiliation{\LIP}
\author{A.~Ankowski} \affiliation{\SLAC}
\author{M.~Antonova} \affiliation{\IFIC}
\author{S.~Antusch} \affiliation{\Basel}
\author{A.~Aranda-Fernandez} \affiliation{\Colima}
\author{A.~Ariga} \affiliation{\Bern}
\author{L.~O.~Arnold} \affiliation{\Columbia}
\author{M.~A.~Arroyave} \affiliation{\EIA}
\author{J.~Asaadi} \affiliation{\TexasArlington}
\author{A.~Aurisano} \affiliation{\Cincinnati}
\author{V.~Aushev} \affiliation{\Kyiv}
\author{D.~Autiero} \affiliation{\IPLyon}
\author{F.~Azfar} \affiliation{\Oxford}
\author{H.~Back} \affiliation{\PacificNorthwest}
\author{J.~J.~Back} \affiliation{\Warwick}
\author{C.~Backhouse} \affiliation{\UniversityCollegeLondon}
\author{P.~Baesso} \affiliation{\Bristol}
\author{L.~Bagby} \affiliation{\Fermi}
\author{R.~Bajou} \affiliation{\Parisuniversite}
\author{S.~Balasubramanian} \affiliation{\Yale}
\author{P.~Baldi} \affiliation{\CalIrvine}
\author{B.~Bambah} \affiliation{\Hyderabad}
\author{F.~Barao} \affiliation{\LIP}\affiliation{\ISTlisboa}
\author{G.~Barenboim} \affiliation{\IFIC}
\author{G.~J.~Barker} \affiliation{\Warwick}
\author{W.~Barkhouse} \affiliation{\Northdakota}
\author{C.~Barnes} \affiliation{\Michigan}
\author{G.~Barr} \affiliation{\Oxford}
\author{J.~Barranco Monarca} \affiliation{\Guanajuato}
\author{N.~Barros} \affiliation{\LIP}\affiliation{\FCULport}
\author{J.~L.~Barrow} \affiliation{\Tennknox}\affiliation{\Fermi}
\author{A.~Bashyal} \affiliation{\OregonState}
\author{V.~Basque} \affiliation{\Manchester}
\author{F.~Bay} \affiliation{\Nikhef}
\author{J.~L.~Bazo~Alba} \affiliation{\Pontificia}
\author{J.~F.~Beacom} \affiliation{\Ohiostate}
\author{E.~Bechetoille} \affiliation{\IPLyon}
\author{B.~Behera} \affiliation{\ColoradoState}
\author{L.~Bellantoni} \affiliation{\Fermi}
\author{G.~Bellettini} \affiliation{\Pisa}
\author{V.~Bellini} \affiliation{\CataniaUniversitadi}\affiliation{\INFNCatania}
\author{O.~Beltramello} \affiliation{\CERN}
\author{D.~Belver} \affiliation{\CIEMAT}
\author{N.~Benekos} \affiliation{\CERN}
\author{F.~Bento Neves} \affiliation{\LIP}
\author{J.~Berger} \affiliation{\Pitt}
\author{S.~Berkman} \affiliation{\Fermi}
\author{P.~Bernardini} \affiliation{\INFNLecce}\affiliation{\Salento}
\author{R.~M.~Berner} \affiliation{\Bern}
\author{H.~Berns} \affiliation{\CalDavis}
\author{S.~Bertolucci} \affiliation{\INFNBologna}\affiliation{\BolognaUniversity}
\author{M.~Betancourt} \affiliation{\Fermi}
\author{Y.~Bezawada} \affiliation{\CalDavis}
\author{M.~Bhattacharjee} \affiliation{\IndGuwahati}
\author{B.~Bhuyan} \affiliation{\IndGuwahati}
\author{S.~Biagi} \affiliation{\INFNSud}
\author{J.~Bian} \affiliation{\CalIrvine}
\author{M.~Biassoni} \affiliation{\INFNMilanBicocca}
\author{K.~Biery} \affiliation{\Fermi}
\author{B.~Bilki} \affiliation{\Beykent}\affiliation{\Iowa}
\author{M.~Bishai} \affiliation{\Brookhaven}
\author{A.~Bitadze} \affiliation{\Manchester}
\author{A.~Blake} \affiliation{\Lancaster}
\author{B.~Blanco Siffert} \affiliation{\FederaldoRio}
\author{F.~D.~M.~Blaszczyk} \affiliation{\Fermi}
\author{G.~C.~Blazey} \affiliation{\Northernillinois}
\author{E.~Blucher} \affiliation{\Chicago}
\author{J.~Boissevain} \affiliation{\LosAlmos}
\author{S.~Bolognesi} \affiliation{\CEASaclay}
\author{T.~Bolton} \affiliation{\Kansasstate}
\author{M.~Bonesini} \affiliation{\INFNMilanBicocca}\affiliation{\MilanoBicocca}
\author{M.~Bongrand} \affiliation{\Lal}
\author{F.~Bonini} \affiliation{\Brookhaven}
\author{A.~Booth} \affiliation{\Sussex}
\author{C.~Booth} \affiliation{\Sheffield}
\author{S.~Bordoni} \affiliation{\CERN}
\author{A.~Borkum} \affiliation{\Sussex}
\author{T.~Boschi} \affiliation{\Durham}
\author{N.~Bostan} \affiliation{\Iowa}
\author{P.~Bour} \affiliation{\CzechTechnical}
\author{S.~B.~Boyd} \affiliation{\Warwick}
\author{D.~Boyden} \affiliation{\Northernillinois}
\author{J.~Bracinik} \affiliation{\Birmingham}
\author{D.~Braga} \affiliation{\Fermi}
\author{D.~Brailsford} \affiliation{\Lancaster}
\author{A.~Brandt} \affiliation{\TexasArlington}
\author{J.~Bremer} \affiliation{\CERN}
\author{C.~Brew} \affiliation{\Rutherford}
\author{E.~Brianne} \affiliation{\Manchester}
\author{S.~J.~Brice} \affiliation{\Fermi}
\author{C.~Brizzolari} \affiliation{\INFNMilanBicocca}\affiliation{\MilanoBicocca}
\author{C.~Bromberg} \affiliation{\Michiganstate}
\author{G.~Brooijmans} \affiliation{\Columbia}
\author{J.~Brooke} \affiliation{\Bristol}
\author{A.~Bross} \affiliation{\Fermi}
\author{G.~Brunetti} \affiliation{\INFNPadova}
\author{N.~Buchanan} \affiliation{\ColoradoState}
\author{H.~Budd} \affiliation{\Rochester}
\author{D.~Caiulo} \affiliation{\IPLyon}
\author{P.~Calafiura} \affiliation{\LawrenceBerkeley}
\author{J.~Calcutt} \affiliation{\Michiganstate}
\author{M.~Calin} \affiliation{\Bucharest}
\author{S.~Calvez} \affiliation{\ColoradoState}
\author{E.~Calvo} \affiliation{\CIEMAT}
\author{L.~Camilleri} \affiliation{\Columbia}
\author{A.~Caminata} \affiliation{\INFNGenova}
\author{M.~Campanelli} \affiliation{\UniversityCollegeLondon}
\author{D.~Caratelli} \affiliation{\Fermi}
\author{G.~Carini} \affiliation{\Brookhaven}
\author{B.~Carlus} \affiliation{\IPLyon}
\author{P.~Carniti} \affiliation{\INFNMilanBicocca}
\author{I.~Caro Terrazas} \affiliation{\ColoradoState}
\author{H.~Carranza} \affiliation{\TexasArlington}
\author{A.~Castillo} \affiliation{\SergioArboleda}
\author{C.~Castromonte} \affiliation{\Ingenieria}
\author{C.~Cattadori} \affiliation{\INFNMilanBicocca}
\author{F.~Cavalier} \affiliation{\Lal}
\author{F.~Cavanna} \affiliation{\Fermi}
\author{S.~Centro} \affiliation{\Padova}
\author{G.~Cerati} \affiliation{\Fermi}
\author{A.~Cervelli} \affiliation{\INFNBologna}
\author{A.~Cervera Villanueva} \affiliation{\IFIC}
\author{M.~Chalifour} \affiliation{\CERN}
\author{C.~Chang} \affiliation{\CalRiverside}
\author{E.~Chardonnet} \affiliation{\Parisuniversite}
\author{N.~Charitonidis} \affiliation{\CERN}
\author{A.~Chatterjee} \affiliation{\Pitt}
\author{S.~Chattopadhyay} \affiliation{\VariableEnergy}
\author{P.~Chatzidaki} \affiliation{\CERN}
\author{J.~Chaves} \affiliation{\Penn}
\author{H.~Chen} \affiliation{\Brookhaven}
\author{M.~Chen} \affiliation{\CalIrvine}
\author{Y.~Chen} \affiliation{\Bern}
\author{D.~Cherdack} \affiliation{\Houston}
\author{C.~Chi} \affiliation{\Columbia}
\author{S.~Childress} \affiliation{\Fermi}
\author{A.~Chiriacescu} \affiliation{\Bucharest}
\author{K.~Cho} \affiliation{\KISTI}
\author{S.~Choubey} \affiliation{\Harish}
\author{A.~Christensen} \affiliation{\ColoradoState}
\author{D.~Christian} \affiliation{\Fermi}
\author{G.~Christodoulou} \affiliation{\CERN}
\author{E.~Church} \affiliation{\PacificNorthwest}
\author{P.~Clarke} \affiliation{\Edinburgh}
\author{T.~E.~Coan} \affiliation{\SouthernMethodist}
\author{A.~G.~Cocco} \affiliation{\INFNNapoli}
\author{J.~A.~B.~Coelho} \affiliation{\Lal}
\author{E.~Conley} \affiliation{\Duke}
\author{J.~M.~Conrad} \affiliation{\Massinsttech}
\author{M.~Convery} \affiliation{\SLAC}
\author{L.~Corwin} \affiliation{\SouthDakotaSchool}
\author{P.~Cotte} \affiliation{\CEASaclay}
\author{L.~Cremaldi} \affiliation{\Mississippi}
\author{L.~Cremonesi} \affiliation{\UniversityCollegeLondon}
\author{J.~I.~Crespo-Anad\'{o}n} \affiliation{\CIEMAT}
\author{E.~Cristaldo} \affiliation{\Asuncion}
\author{R.~Cross} \affiliation{\Lancaster}
\author{C.~Cuesta} \affiliation{\CIEMAT}
\author{Y.~Cui} \affiliation{\CalRiverside}
\author{D.~Cussans} \affiliation{\Bristol}
\author{M.~Dabrowski} \affiliation{\Brookhaven}
\author{H.~da Motta} \affiliation{\CBPF}
\author{L.~Da Silva Peres} \affiliation{\FederaldoRio}
\author{C.~David} \affiliation{\Fermi}\affiliation{\York}
\author{Q.~David} \affiliation{\IPLyon}
\author{G.~S.~Davies} \affiliation{\Mississippi}
\author{S.~Davini} \affiliation{\INFNGenova}
\author{J.~Dawson} \affiliation{\Parisuniversite}
\author{K.~De} \affiliation{\TexasArlington}
\author{R.~M.~De Almeida} \affiliation{\Fluminense}
\author{P.~Debbins} \affiliation{\Iowa}
\author{I.~De Bonis} \affiliation{\DannecyleVieux}
\author{M.~P.~Decowski} \affiliation{\Nikhef}\affiliation{\Amsterdam}
\author{A.~de Gouv\^ea} \affiliation{\Northwestern}
\author{P.~C.~De Holanda} \affiliation{\Campinas}
\author{I.~L.~De Icaza Astiz} \affiliation{\Sussex}
\author{A.~Deisting} \affiliation{\Royalholloway}
\author{P.~De Jong} \affiliation{\Nikhef}\affiliation{\Amsterdam}
\author{A.~Delbart} \affiliation{\CEASaclay}
\author{D.~Delepine} \affiliation{\Guanajuato}
\author{M.~Delgado} \affiliation{\AntonioNarino}
\author{A.~Dell’Acqua} \affiliation{\CERN}
\author{P.~De Lurgio} \affiliation{\Argonne}
\author{J.~R.~T.~de Mello Neto} \affiliation{\FederaldoRio}
\author{D.~M.~DeMuth} \affiliation{\ValleyCity}
\author{S.~Dennis} \affiliation{\Cambridge}
\author{C.~Densham} \affiliation{\Rutherford}
\author{G.~Deptuch} \affiliation{\Fermi}
\author{A.~De Roeck} \affiliation{\CERN}
\author{V.~De Romeri} \affiliation{\IFIC}
\author{J.~J.~De Vries} \affiliation{\Cambridge}
\author{R.~Dharmapalan} \affiliation{\Hawaii}
\author{M.~Dias} \affiliation{\Unifesp}
\author{F.~Diaz} \affiliation{\Pontificia}
\author{J.~S.~D\'iaz} \affiliation{\Indiana}
\author{S.~Di Domizio} \affiliation{\INFNGenova}\affiliation{\Genova}
\author{L.~Di Giulio} \affiliation{\CERN}
\author{P.~Ding} \affiliation{\Fermi}
\author{L.~Di Noto} \affiliation{\INFNGenova}\affiliation{\Genova}
\author{C.~Distefano} \affiliation{\INFNSud}
\author{R.~Diurba} \affiliation{\Minntwin}
\author{M.~Diwan} \affiliation{\Brookhaven}
\author{Z.~Djurcic} \affiliation{\Argonne}
\author{N.~Dokania} \affiliation{\StonyBrook}
\author{M.~J.~Dolinski} \affiliation{\Drexel}
\author{L.~Domine} \affiliation{\SLAC}
\author{D.~Douglas} \affiliation{\Michiganstate}
\author{F.~Drielsma} \affiliation{\SLAC}
\author{D.~Duchesneau} \affiliation{\DannecyleVieux}
\author{K.~Duffy} \affiliation{\Fermi}
\author{P.~Dunne} \affiliation{\Imperial}
\author{T.~Durkin} \affiliation{\Rutherford}
\author{H.~Duyang} \affiliation{\Southcarolina}
\author{O.~Dvornikov} \affiliation{\Hawaii}
\author{D.~A.~Dwyer} \affiliation{\LawrenceBerkeley}
\author{A.~S.~Dyshkant} \affiliation{\Northernillinois}
\author{M.~Eads} \affiliation{\Northernillinois}
\author{D.~Edmunds} \affiliation{\Michiganstate}
\author{J.~Eisch} \affiliation{\IowaState}
\author{S.~Emery} \affiliation{\CEASaclay}
\author{A.~Ereditato} \affiliation{\Bern}
\author{C.~O.~Escobar} \affiliation{\Fermi}
\author{L.~Escudero Sanchez} \affiliation{\Cambridge}
\author{J.~J.~Evans} \affiliation{\Manchester}
\author{E.~Ewart} \affiliation{\Indiana}
\author{A.~C.~Ezeribe} \affiliation{\Sheffield}
\author{C.~Fabre} \affiliation{\CERN}
\author{K.~Fahey} \affiliation{\Fermi}
\author{A.~Falcone} \affiliation{\INFNMilanBicocca}\affiliation{\MilanoBicocca}
\author{C.~Farnese} \affiliation{\Padova}
\author{Y.~Farzan} \affiliation{\IPM}
\author{J.~Felix} \affiliation{\Guanajuato}
\author{E.~Fernandez-Martinez} \affiliation{\Madrid}
\author{P.~Fernandez Menendez} \affiliation{\IFIC}
\author{F.~Ferraro} \affiliation{\INFNGenova}\affiliation{\Genova}
\author{L.~Fields} \affiliation{\Fermi}
\author{A.~Filkins} \affiliation{\WilliamMary}
\author{F.~Filthaut} \affiliation{\Nikhef}\affiliation{\Radboud}
\author{R.~S.~Fitzpatrick} \affiliation{\Michigan}
\author{W.~Flanagan} \affiliation{\Dallas}
\author{B.~Fleming} \affiliation{\Yale}
\author{R.~Flight} \affiliation{\Rochester}
\author{J.~Fowler} \affiliation{\Duke}
\author{W.~Fox} \affiliation{\Indiana}
\author{J.~Franc} \affiliation{\CzechTechnical}
\author{K.~Francis} \affiliation{\Northernillinois}
\author{D.~Franco} \affiliation{\Yale}
\author{J.~Freeman} \affiliation{\Fermi}
\author{J.~Freestone} \affiliation{\Manchester}
\author{J.~Fried} \affiliation{\Brookhaven}
\author{A.~Friedland} \affiliation{\SLAC}
\author{S.~Fuess} \affiliation{\Fermi}
\author{I.~Furic} \affiliation{\Florida}
\author{A.~P.~Furmanski} \affiliation{\Minntwin}
\author{A.~Gago} \affiliation{\Pontificia}
\author{H.~Gallagher} \affiliation{\Tufts}
\author{A.~Gallego-Ros} \affiliation{\CIEMAT}
\author{N.~Gallice} \affiliation{\INFNMilano}\affiliation{\MilanoUniv}
\author{V.~Galymov} \affiliation{\IPLyon}
\author{E.~Gamberini} \affiliation{\CERN}
\author{T.~Gamble} \affiliation{\Sheffield}
\author{R.~Gandhi} \affiliation{\Harish}
\author{R.~Gandrajula} \affiliation{\Michiganstate}
\author{S.~Gao} \affiliation{\Brookhaven}
\author{D.~Garcia-Gamez} \affiliation{\Granada}
\author{M.~\'{A}.~Garc\'ia-Peris} \affiliation{\IFIC}
\author{S.~Gardiner} \affiliation{\Fermi}
\author{D.~Gastler} \affiliation{\Boston}
\author{G.~Ge} \affiliation{\Columbia}
\author{B.~Gelli} \affiliation{\Campinas}
\author{A.~Gendotti} \affiliation{\ETH}
\author{S.~Gent} \affiliation{\SouthDakotaState}
\author{Z.~Ghorbani-Moghaddam} \affiliation{\INFNGenova}
\author{D.~Gibin} \affiliation{\Padova}
\author{I.~Gil-Botella} \affiliation{\CIEMAT}
\author{C.~Girerd} \affiliation{\IPLyon}
\author{A.~K.~Giri} \affiliation{\IndHyderabad}
\author{D.~Gnani} \affiliation{\LawrenceBerkeley}
\author{O.~Gogota} \affiliation{\Kyiv}
\author{M.~Gold} \affiliation{\Newmexico}
\author{S.~Gollapinni} \affiliation{\LosAlmos}
\author{K.~Gollwitzer} \affiliation{\Fermi}
\author{R.~A.~Gomes} \affiliation{\FederaldeGoias}
\author{L.~V.~Gomez Bermeo} \affiliation{\SergioArboleda}
\author{L.~S.~Gomez Fajardo} \affiliation{\SergioArboleda}
\author{F.~Gonnella} \affiliation{\Birmingham}
\author{J.~A.~Gonzalez-Cuevas} \affiliation{\Asuncion}
\author{M.~C.~Goodman} \affiliation{\Argonne}
\author{O.~Goodwin} \affiliation{\Manchester}
\author{S.~Goswami} \affiliation{\PhysicalResearchLaboratory}
\author{C.~Gotti} \affiliation{\INFNMilanBicocca}
\author{E.~Goudzovski} \affiliation{\Birmingham}
\author{C.~Grace} \affiliation{\LawrenceBerkeley}
\author{M.~Graham} \affiliation{\SLAC}
\author{E.~Gramellini} \affiliation{\Yale}
\author{R.~Gran} \affiliation{\Minnduluth}
\author{E.~Granados} \affiliation{\Guanajuato}
\author{A.~Grant} \affiliation{\Daresbury}
\author{C.~Grant} \affiliation{\Boston}
\author{D.~Gratieri} \affiliation{\Fluminense}
\author{P.~Green} \affiliation{\Manchester}
\author{S.~Green} \affiliation{\Cambridge}
\author{L.~Greenler} \affiliation{\Wisconsin}
\author{M.~Greenwood} \affiliation{\OregonState}
\author{J.~Greer} \affiliation{\Bristol}
\author{W.~C.~Griffith} \affiliation{\Sussex}
\author{M.~Groh} \affiliation{\Indiana}
\author{J.~Grudzinski} \affiliation{\Argonne}
\author{K.~Grzelak} \affiliation{\Warsaw}
\author{W.~Gu} \affiliation{\Brookhaven}
\author{V.~Guarino} \affiliation{\Argonne}
\author{R.~Guenette} \affiliation{\Harvard}
\author{A.~Guglielmi} \affiliation{\INFNPadova}
\author{B.~Guo} \affiliation{\Southcarolina}
\author{K.~K.~Guthikonda} \affiliation{\KL}
\author{R.~Gutierrez} \affiliation{\AntonioNarino}
\author{P.~Guzowski} \affiliation{\Manchester}
\author{M.~M.~Guzzo} \affiliation{\Campinas}
\author{S.~Gwon} \affiliation{\ChungAng}
\author{K.~Haaf} \affiliation{\Fermi}
\author{A.~Habig} \affiliation{\Minnduluth}
\author{A.~Hackenburg} \affiliation{\Yale}
\author{H.~Hadavand} \affiliation{\TexasArlington}
\author{R.~Haenni} \affiliation{\Bern}
\author{A.~Hahn} \affiliation{\Fermi}
\author{J.~Haigh} \affiliation{\Warwick}
\author{J.~Haiston} \affiliation{\SouthDakotaSchool}
\author{T.~Hamernik} \affiliation{\Fermi}
\author{P.~Hamilton} \affiliation{\Imperial}
\author{J.~Han} \affiliation{\Pitt}
\author{K.~Harder} \affiliation{\Rutherford}
\author{D.~A.~Harris} \affiliation{\Fermi}\affiliation{\York}
\author{J.~Hartnell} \affiliation{\Sussex}
\author{T.~Hasegawa} \affiliation{\KEK}
\author{R.~Hatcher} \affiliation{\Fermi}
\author{E.~Hazen} \affiliation{\Boston}
\author{A.~Heavey} \affiliation{\Fermi}
\author{K.~M.~Heeger} \affiliation{\Yale}
\author{J.~Heise} \affiliation{\SURF}
\author{K.~Hennessy} \affiliation{\Liverpool}
\author{S.~Henry} \affiliation{\Rochester}
\author{M.~A.~Hernandez Morquecho} \affiliation{\Guanajuato}
\author{K.~Herner} \affiliation{\Fermi}
\author{L.~Hertel} \affiliation{\CalIrvine}
\author{A.~S.~Hesam} \affiliation{\CERN}
\author{J.~Hewes} \affiliation{\Cincinnati}
\author{A.~Higuera} \affiliation{\Houston}
\author{T.~Hill} \affiliation{\Idaho}
\author{S.~J.~Hillier} \affiliation{\Birmingham}
\author{A.~Himmel} \affiliation{\Fermi}
\author{J.~Hoff} \affiliation{\Fermi}
\author{C.~Hohl} \affiliation{\Basel}
\author{A.~Holin} \affiliation{\UniversityCollegeLondon}
\author{E.~Hoppe} \affiliation{\PacificNorthwest}
\author{G.~A.~Horton-Smith} \affiliation{\Kansasstate}
\author{M.~Hostert} \affiliation{\Durham}
\author{A.~Hourlier} \affiliation{\Massinsttech}
\author{B.~Howard} \affiliation{\Fermi}
\author{R.~Howell} \affiliation{\Rochester}
\author{J.~Hrivnak} \affiliation{\CERN}
\author{J.~Huang} \affiliation{\Texasaustin}
\author{J.~Huang} \affiliation{\CalDavis}
\author{J.~Hugon} \affiliation{\Louisanastate}
\author{G.~Iles} \affiliation{\Imperial}
\author{N.~Ilic} \affiliation{\Toronto}
\author{A.~M.~Iliescu} \affiliation{\INFNBologna}
\author{R.~Illingworth} \affiliation{\Fermi}
\author{A.~Ioannisian} \affiliation{\Yerevan}
\author{R.~Itay} \affiliation{\SLAC}
\author{A.~Izmaylov} \affiliation{\IFIC}
\author{E.~James} \affiliation{\Fermi}
\author{B.~Jargowsky} \affiliation{\CalIrvine}
\author{F.~Jediny} \affiliation{\CzechTechnical}
\author{C.~Jes\`{u}s-Valls} \affiliation{\IFAE}
\author{X.~Ji} \affiliation{\Brookhaven}
\author{L.~Jiang} \affiliation{\VirginiaTech}
\author{S.~Jim\'{e}nez} \affiliation{\CIEMAT}
\author{A.~Jipa} \affiliation{\Bucharest}
\author{A.~Joglekar} \affiliation{\CalRiverside}
\author{C.~Johnson} \affiliation{\ColoradoState}
\author{R.~Johnson} \affiliation{\Cincinnati}
\author{B.~Jones} \affiliation{\TexasArlington}
\author{S.~Jones} \affiliation{\UniversityCollegeLondon}
\author{C.~K.~Jung} \affiliation{\StonyBrook}
\author{T.~Junk} \affiliation{\Fermi}
\author{Y.~Jwa} \affiliation{\Columbia}
\author{M.~Kabirnezhad} \affiliation{\Oxford}
\author{A.~Kaboth} \affiliation{\Rutherford}
\author{I.~Kadenko} \affiliation{\Kyiv}
\author{F.~Kamiya} \affiliation{\FederaldoABC}
\author{G.~Karagiorgi} \affiliation{\Columbia}
\author{A.~Karcher} \affiliation{\LawrenceBerkeley}
\author{M.~Karolak} \affiliation{\CEASaclay}
\author{Y.~Karyotakis} \affiliation{\DannecyleVieux}
\author{S.~Kasai} \affiliation{\Kure}
\author{S.~P.~Kasetti} \affiliation{\Louisanastate}
\author{L.~Kashur} \affiliation{\ColoradoState}
\author{N.~Kazaryan} \affiliation{\Yerevan}
\author{E.~Kearns} \affiliation{\Boston}
\author{P.~Keener} \affiliation{\Penn}
\author{K.~J.~Kelly} \affiliation{\Fermi}
\author{E.~Kemp} \affiliation{\Campinas}
\author{C.~Kendziora} \affiliation{\Fermi}
\author{W.~Ketchum} \affiliation{\Fermi}
\author{S.~H.~Kettell} \affiliation{\Brookhaven}
\author{M.~Khabibullin} \affiliation{\INR}
\author{A.~Khotjantsev} \affiliation{\INR}
\author{A.~Khvedelidze} \affiliation{\Georgian}
\author{D.~Kim} \affiliation{\CERN}
\author{B.~King} \affiliation{\Fermi}
\author{B.~Kirby} \affiliation{\Brookhaven}
\author{M.~Kirby} \affiliation{\Fermi}
\author{J.~Klein} \affiliation{\Penn}
\author{K.~Koehler} \affiliation{\Wisconsin}
\author{L.~W.~Koerner} \affiliation{\Houston}
\author{S.~Kohn} \affiliation{\CalBerkeley}\affiliation{\LawrenceBerkeley}
\author{P.~P.~Koller} \affiliation{\Bern}
\author{M.~Kordosky} \affiliation{\WilliamMary}
\author{T.~Kosc} \affiliation{\IPLyon}
\author{U.~Kose} \affiliation{\CERN}
\author{V.~A.~Kosteleck\'y} \affiliation{\Indiana}
\author{K.~Kothekar} \affiliation{\Bristol}
\author{F.~Krennrich} \affiliation{\IowaState}
\author{I.~Kreslo} \affiliation{\Bern}
\author{Y.~Kudenko} \affiliation{\INR}
\author{V.~A.~Kudryavtsev} \affiliation{\Sheffield}
\author{S.~Kulagin} \affiliation{\INR}
\author{J.~Kumar} \affiliation{\Hawaii}
\author{R.~Kumar} \affiliation{\Punjab}
\author{C.~Kuruppu} \affiliation{\Southcarolina}
\author{V.~Kus} \affiliation{\CzechTechnical}
\author{T.~Kutter} \affiliation{\Louisanastate}
\author{B.~Lacarelle} \affiliation{\CERN}
\author{A.~Lambert} \affiliation{\LawrenceBerkeley}
\author{K.~Lande} \affiliation{\Penn}
\author{C.~E.~Lane} \affiliation{\Drexel}
\author{K.~Lang} \affiliation{\Texasaustin}
\author{T.~Langford} \affiliation{\Yale}
\author{P.~Lasorak} \affiliation{\Sussex}
\author{D.~Last} \affiliation{\Penn}
\author{C.~Lastoria} \affiliation{\CIEMAT}
\author{A.~Laundrie} \affiliation{\Wisconsin}
\author{A.~Lawrence} \affiliation{\LawrenceBerkeley}
\author{I.~Lazanu} \affiliation{\Bucharest}
\author{R.~LaZur} \affiliation{\ColoradoState}
\author{T.~Le} \affiliation{\Tufts}
\author{J.~Learned} \affiliation{\Hawaii}
\author{P.~LeBrun} \affiliation{\IPLyon}
\author{G.~Lehmann Miotto} \affiliation{\CERN}
\author{R.~Lehnert} \affiliation{\Indiana}
\author{M.~A.~Leigui de Oliveira} \affiliation{\FederaldoABC}
\author{M.~Leitner} \affiliation{\LawrenceBerkeley}
\author{M.~Leyton} \affiliation{\IFAE}
\author{L.~Li} \affiliation{\CalIrvine}
\author{S.~Li} \affiliation{\Brookhaven}
\author{S.~W.~Li} \affiliation{\SLAC}
\author{T.~Li} \affiliation{\Edinburgh}
\author{Y.~Li} \affiliation{\Brookhaven}
\author{H.~Liao} \affiliation{\Kansasstate}
\author{C.~S.~Lin} \affiliation{\LawrenceBerkeley}
\author{S.~Lin} \affiliation{\Louisanastate}
\author{A.~Lister} \affiliation{\Wisconsin}
\author{B.~R.~Littlejohn} \affiliation{\Illinoisinstitute}
\author{J.~Liu} \affiliation{\CalIrvine}
\author{T.~Liu} \affiliation{\Chicago}
\author{S.~Lockwitz} \affiliation{\Fermi}
\author{T.~Loew} \affiliation{\LawrenceBerkeley}
\author{M.~Lokajicek} \affiliation{\CzechAcademyofSciences}
\author{I.~Lomidze} \affiliation{\Georgian}
\author{K.~Long} \affiliation{\Imperial}
\author{K.~Loo} \affiliation{\Jyvaskyla}
\author{D.~Lorca} \affiliation{\Bern}
\author{T.~Lord} \affiliation{\Warwick}
\author{J.~M.~LoSecco} \affiliation{\NotreDame}
\author{W.~C.~Louis} \affiliation{\LosAlmos}
\author{K.B.~Luk} \affiliation{\CalBerkeley}\affiliation{\LawrenceBerkeley}
\author{X.~Luo} \affiliation{\CalSantabarbara}
\author{N.~Lurkin} \affiliation{\Birmingham}
\author{T.~Lux} \affiliation{\IFAE}
\author{V.~P.~Luzio} \affiliation{\FederaldoABC}
\author{D.~MacFarland} \affiliation{\SLAC}
\author{A.~A.~Machado} \affiliation{\Campinas}
\author{P.~Machado} \affiliation{\Fermi}
\author{C.~T.~Macias} \affiliation{\Indiana}
\author{J.~R.~Macier} \affiliation{\Fermi}
\author{A.~Maddalena} \affiliation{\GranSassoLab}
\author{P.~Madigan} \affiliation{\CalBerkeley}\affiliation{\LawrenceBerkeley}
\author{S.~Magill} \affiliation{\Argonne}
\author{K.~Mahn} \affiliation{\Michiganstate}
\author{A.~Maio} \affiliation{\LIP}\affiliation{\FCULport}
\author{J.~A.~Maloney} \affiliation{\DakotaState}
\author{G.~Mandrioli} \affiliation{\INFNBologna}
\author{J.~Maneira} \affiliation{\LIP}\affiliation{\FCULport}
\author{L.~Manenti} \affiliation{\UniversityCollegeLondon}
\author{S.~Manly} \affiliation{\Rochester}
\author{A.~Mann} \affiliation{\Tufts}
\author{K.~Manolopoulos} \affiliation{\Rutherford}
\author{M.~Manrique Plata} \affiliation{\Indiana}
\author{A.~Marchionni} \affiliation{\Fermi}
\author{W.~Marciano} \affiliation{\Brookhaven}
\author{D.~Marfatia} \affiliation{\Hawaii}
\author{C.~Mariani} \affiliation{\VirginiaTech}
\author{J.~Maricic} \affiliation{\Hawaii}
\author{F.~Marinho} \affiliation{\FederaldeSaoCarlos}
\author{A.~D.~Marino} \affiliation{\ColoradoBoulder}
\author{M.~Marshak} \affiliation{\Minntwin}
\author{C.~Marshall} \affiliation{\LawrenceBerkeley}
\author{J.~Marshall} \affiliation{\Warwick}
\author{J.~Marteau} \affiliation{\IPLyon}
\author{J.~Martin-Albo} \affiliation{\IFIC}
\author{N.~Martinez} \affiliation{\Kansasstate}
\author{D.A.~Martinez Caicedo } \affiliation{\SouthDakotaSchool}
\author{S.~Martynenko} \affiliation{\StonyBrook}
\author{K.~Mason} \affiliation{\Tufts}
\author{A.~Mastbaum} \affiliation{\Rutgers}
\author{M.~Masud} \affiliation{\IFIC}
\author{S.~Matsuno} \affiliation{\Hawaii}
\author{J.~Matthews} \affiliation{\Louisanastate}
\author{C.~Mauger} \affiliation{\Penn}
\author{N.~Mauri} \affiliation{\INFNBologna}\affiliation{\BolognaUniversity}
\author{K.~Mavrokoridis} \affiliation{\Liverpool}
\author{R.~Mazza} \affiliation{\INFNMilanBicocca}
\author{A.~Mazzacane} \affiliation{\Fermi}
\author{E.~Mazzucato} \affiliation{\CEASaclay}
\author{E.~McCluskey} \affiliation{\Fermi}
\author{N.~McConkey} \affiliation{\Manchester}
\author{K.~S.~McFarland} \affiliation{\Rochester}
\author{C.~McGrew} \affiliation{\StonyBrook}
\author{A.~McNab} \affiliation{\Manchester}
\author{A.~Mefodiev} \affiliation{\INR}
\author{P.~Mehta} \affiliation{\Jawaharlal}
\author{P.~Melas} \affiliation{\Athens}
\author{M.~Mellinato} \affiliation{\INFNMilanBicocca}\affiliation{\MilanoBicocca}
\author{O.~Mena} \affiliation{\IFIC}
\author{S.~Menary} \affiliation{\York}
\author{H.~Mendez} \affiliation{\PuertoRico}
\author{A.~Menegolli} \affiliation{\INFNPavia}\affiliation{\Pavia}
\author{G.~Meng} \affiliation{\INFNPadova}
\author{M.~D.~Messier} \affiliation{\Indiana}
\author{W.~Metcalf} \affiliation{\Louisanastate}
\author{M.~Mewes} \affiliation{\Indiana}
\author{H.~Meyer} \affiliation{\Wichita}
\author{T.~Miao} \affiliation{\Fermi}
\author{G.~Michna} \affiliation{\SouthDakotaState}
\author{T.~Miedema} \affiliation{\Nikhef}\affiliation{\Radboud}
\author{J.~Migenda} \affiliation{\Sheffield}
\author{R.~Milincic} \affiliation{\Hawaii}
\author{W.~Miller} \affiliation{\Minntwin}
\author{J.~Mills} \affiliation{\Tufts}
\author{C.~Milne} \affiliation{\Idaho}
\author{O.~Mineev} \affiliation{\INR}
\author{O.~G.~Miranda} \affiliation{\Cinvestav}
\author{S.~Miryala} \affiliation{\Brookhaven}
\author{C.~S.~Mishra} \affiliation{\Fermi}
\author{S.~R.~Mishra} \affiliation{\Southcarolina}
\author{A.~Mislivec} \affiliation{\Minntwin}
\author{D.~Mladenov} \affiliation{\CERN}
\author{I.~Mocioiu} \affiliation{\PennState}
\author{K.~Moffat} \affiliation{\Durham}
\author{N.~Moggi} \affiliation{\INFNBologna}\affiliation{\BolognaUniversity}
\author{R.~Mohanta} \affiliation{\Hyderabad}
\author{T.~A.~Mohayai} \affiliation{\Fermi}
\author{N.~Mokhov} \affiliation{\Fermi}
\author{J.~Molina} \affiliation{\Asuncion}
\author{L.~Molina Bueno} \affiliation{\ETH}
\author{A.~Montanari} \affiliation{\INFNBologna}
\author{C.~Montanari} \affiliation{\INFNPavia}\affiliation{\Pavia}
\author{D.~Montanari} \affiliation{\Fermi}
\author{L.~M.~Montano Zetina} \affiliation{\Cinvestav}
\author{J.~Moon} \affiliation{\Massinsttech}
\author{M.~Mooney} \affiliation{\ColoradoState}
\author{A.~Moor} \affiliation{\Cambridge}
\author{D.~Moreno} \affiliation{\AntonioNarino}
\author{B.~Morgan} \affiliation{\Warwick}
\author{C.~Morris} \affiliation{\Houston}
\author{C.~Mossey} \affiliation{\Fermi}
\author{E.~Motuk} \affiliation{\UniversityCollegeLondon}
\author{C.~A.~Moura} \affiliation{\FederaldoABC}
\author{J.~Mousseau} \affiliation{\Michigan}
\author{W.~Mu} \affiliation{\Fermi}
\author{L.~Mualem} \affiliation{\Caltech}
\author{J.~Mueller} \affiliation{\ColoradoState}
\author{M.~Muether} \affiliation{\Wichita}
\author{S.~Mufson} \affiliation{\Indiana}
\author{F.~Muheim} \affiliation{\Edinburgh}
\author{A.~Muir} \affiliation{\Daresbury}
\author{M.~Mulhearn} \affiliation{\CalDavis}
\author{H.~Muramatsu} \affiliation{\Minntwin}
\author{S.~Murphy} \affiliation{\ETH}
\author{J.~Musser} \affiliation{\Indiana}
\author{J.~Nachtman} \affiliation{\Iowa}
\author{S.~Nagu} \affiliation{\Lucknow}
\author{M.~Nalbandyan} \affiliation{\Yerevan}
\author{R.~Nandakumar} \affiliation{\Rutherford}
\author{D.~Naples} \affiliation{\Pitt}
\author{S.~Narita} \affiliation{\Iwate}
\author{D.~Navas-Nicol\'{a}s} \affiliation{\CIEMAT}
\author{N.~Nayak} \affiliation{\CalIrvine}
\author{M.~Nebot-Guinot} \affiliation{\Edinburgh}
\author{L.~Necib} \affiliation{\Caltech}
\author{K.~Negishi} \affiliation{\Iwate}
\author{J.~K.~Nelson} \affiliation{\WilliamMary}
\author{J.~Nesbit} \affiliation{\Wisconsin}
\author{M.~Nessi} \affiliation{\CERN}
\author{D.~Newbold} \affiliation{\Rutherford}
\author{M.~Newcomer} \affiliation{\Penn}
\author{D.~Newhart} \affiliation{\Fermi}
\author{R.~Nichol} \affiliation{\UniversityCollegeLondon}
\author{E.~Niner} \affiliation{\Fermi}
\author{K.~Nishimura} \affiliation{\Hawaii}
\author{A.~Norman} \affiliation{\Fermi}
\author{A.~Norrick} \affiliation{\Fermi}
\author{R.~Northrop} \affiliation{\Chicago}
\author{P.~Novella} \affiliation{\IFIC}
\author{J.~A.~Nowak} \affiliation{\Lancaster}
\author{M.~Oberling} \affiliation{\Argonne}
\author{A.~Olivares Del Campo} \affiliation{\Durham}
\author{A.~Olivier} \affiliation{\Rochester}
\author{Y.~Onel} \affiliation{\Iowa}
\author{Y.~Onishchuk} \affiliation{\Kyiv}
\author{J.~Ott} \affiliation{\CalIrvine}
\author{L.~Pagani} \affiliation{\CalDavis}
\author{S.~Pakvasa} \affiliation{\Hawaii}
\author{O.~Palamara} \affiliation{\Fermi}
\author{S.~Palestini} \affiliation{\CERN}
\author{J.~M.~Paley} \affiliation{\Fermi}
\author{M.~Pallavicini} \affiliation{\INFNGenova}\affiliation{\Genova}
\author{C.~Palomares} \affiliation{\CIEMAT}
\author{E.~Pantic} \affiliation{\CalDavis}
\author{V.~Paolone} \affiliation{\Pitt}
\author{V.~Papadimitriou} \affiliation{\Fermi}
\author{R.~Papaleo} \affiliation{\INFNSud}
\author{A.~Papanestis} \affiliation{\Rutherford}
\author{S.~Paramesvaran} \affiliation{\Bristol}
\author{S.~Parke} \affiliation{\Fermi}
\author{Z.~Parsa} \affiliation{\Brookhaven}
\author{M.~Parvu} \affiliation{\Bucharest}
\author{S.~Pascoli} \affiliation{\Durham}
\author{L.~Pasqualini} \affiliation{\INFNBologna}\affiliation{\BolognaUniversity}
\author{J.~Pasternak} \affiliation{\Imperial}
\author{J.~Pater} \affiliation{\Manchester}
\author{C.~Patrick} \affiliation{\UniversityCollegeLondon}
\author{L.~Patrizii} \affiliation{\INFNBologna}
\author{R.~B.~Patterson} \affiliation{\Caltech}
\author{S.~J.~Patton} \affiliation{\LawrenceBerkeley}
\author{T.~Patzak} \affiliation{\Parisuniversite}
\author{A.~Paudel} \affiliation{\Kansasstate}
\author{B.~Paulos} \affiliation{\Wisconsin}
\author{L.~Paulucci} \affiliation{\FederaldoABC}
\author{Z.~Pavlovic} \affiliation{\Fermi}
\author{G.~Pawloski} \affiliation{\Minntwin}
\author{D.~Payne} \affiliation{\Liverpool}
\author{V.~Pec} \affiliation{\Sheffield}
\author{S.~J.~M.~Peeters} \affiliation{\Sussex}
\author{Y.~Penichot} \affiliation{\CEASaclay}
\author{E.~Pennacchio} \affiliation{\IPLyon}
\author{A.~Penzo} \affiliation{\Iowa}
\author{O.~L.~G.~Peres} \affiliation{\Campinas}
\author{J.~Perry} \affiliation{\Edinburgh}
\author{D.~Pershey} \affiliation{\Duke}
\author{G.~Pessina} \affiliation{\INFNMilanBicocca}
\author{G.~Petrillo} \affiliation{\SLAC}
\author{C.~Petta} \affiliation{\CataniaUniversitadi}\affiliation{\INFNCatania}
\author{R.~Petti} \affiliation{\Southcarolina}
\author{F.~Piastra} \affiliation{\Bern}
\author{L.~Pickering} \affiliation{\Michiganstate}
\author{F.~Pietropaolo} \affiliation{\CERN}\affiliation{\INFNPadova}
\author{J.~Pillow} \affiliation{\Warwick}
\author{J.~Pinzino} \affiliation{\Toronto}
\author{R.~Plunkett} \affiliation{\Fermi}
\author{R.~Poling} \affiliation{\Minntwin}
\author{X.~Pons} \affiliation{\CERN}
\author{N.~Poonthottathil} \affiliation{\IowaState}
\author{S.~Pordes} \affiliation{\Fermi}
\author{M.~Potekhin} \affiliation{\Brookhaven}
\author{R.~Potenza} \affiliation{\CataniaUniversitadi}\affiliation{\INFNCatania}
\author{B.~V.~K.~S.~Potukuchi} \affiliation{\Jammu}
\author{J.~Pozimski} \affiliation{\Imperial}
\author{M.~Pozzato} \affiliation{\INFNBologna}\affiliation{\BolognaUniversity}
\author{S.~Prakash} \affiliation{\Campinas}
\author{T.~Prakash} \affiliation{\LawrenceBerkeley}
\author{S.~Prince} \affiliation{\Harvard}
\author{G.~Prior} \affiliation{\LIP}
\author{D.~Pugnere} \affiliation{\IPLyon}
\author{K.~Qi} \affiliation{\StonyBrook}
\author{X.~Qian} \affiliation{\Brookhaven}
\author{J.~L.~Raaf} \affiliation{\Fermi}
\author{R.~Raboanary} \affiliation{\Antananarivo}
\author{V.~Radeka} \affiliation{\Brookhaven}
\author{J.~Rademacker} \affiliation{\Bristol}
\author{B.~Radics} \affiliation{\ETH}
\author{A.~Rafique} \affiliation{\Argonne}
\author{E.~Raguzin} \affiliation{\Brookhaven}
\author{M.~Rai} \affiliation{\Warwick}
\author{M.~Rajaoalisoa} \affiliation{\Cincinnati}
\author{I.~Rakhno} \affiliation{\Fermi}
\author{H.~T.~Rakotondramanana} \affiliation{\Antananarivo}
\author{L.~Rakotondravohitra} \affiliation{\Antananarivo}
\author{Y.~A.~Ramachers} \affiliation{\Warwick}
\author{R.~Rameika} \affiliation{\Fermi}
\author{M.~A.~Ramirez Delgado} \affiliation{\Guanajuato}
\author{B.~Ramson} \affiliation{\Fermi}
\author{A.~Rappoldi} \affiliation{\INFNPavia}\affiliation{\Pavia}
\author{G.~Raselli} \affiliation{\INFNPavia}\affiliation{\Pavia}
\author{P.~Ratoff} \affiliation{\Lancaster}
\author{S.~Ravat} \affiliation{\CERN}
\author{H.~Razafinime} \affiliation{\Antananarivo}
\author{J.~S.~Real} \affiliation{\Grenoble}
\author{B.~Rebel} \affiliation{\Wisconsin}\affiliation{\Fermi}
\author{D.~Redondo} \affiliation{\CIEMAT}
\author{M.~Reggiani-Guzzo} \affiliation{\Campinas}
\author{T.~Rehak} \affiliation{\Drexel}
\author{J.~Reichenbacher} \affiliation{\SouthDakotaSchool}
\author{S.~D.~Reitzner} \affiliation{\Fermi}
\author{A.~Renshaw} \affiliation{\Houston}
\author{S.~Rescia} \affiliation{\Brookhaven}
\author{F.~Resnati} \affiliation{\CERN}
\author{A.~Reynolds} \affiliation{\Oxford}
\author{G.~Riccobene} \affiliation{\INFNSud}
\author{L.~C.~J.~Rice} \affiliation{\Pitt}
\author{K.~Rielage} \affiliation{\LosAlmos}
\author{A.~Rigamonti} \affiliation{\CERN}
\author{Y.~Rigaut} \affiliation{\ETH}
\author{D.~Rivera} \affiliation{\Penn}
\author{L.~Rochester} \affiliation{\SLAC}
\author{M.~Roda} \affiliation{\Liverpool}
\author{P.~Rodrigues} \affiliation{\Oxford}
\author{M.~J.~Rodriguez Alonso} \affiliation{\CERN}
\author{J.~Rodriguez Rondon} \affiliation{\SouthDakotaSchool}
\author{A.~J.~Roeth} \affiliation{\Duke}
\author{H.~Rogers} \affiliation{\ColoradoState}
\author{S.~Rosauro-Alcaraz} \affiliation{\Madrid}
\author{M.~Rosenthal} \affiliation{\CERN}
\author{M.~Rossella} \affiliation{\INFNPavia}\affiliation{\Pavia}
\author{J.~Rout} \affiliation{\Jawaharlal}
\author{S.~Roy} \affiliation{\Harish}
\author{A.~Rubbia} \affiliation{\ETH}
\author{C.~Rubbia} \affiliation{\GranSasso}
\author{B.~Russell} \affiliation{\LawrenceBerkeley}
\author{J.~Russell} \affiliation{\SLAC}
\author{D.~Ruterbories} \affiliation{\Rochester}
\author{R.~Saakyan} \affiliation{\UniversityCollegeLondon}
\author{S.~Sacerdoti} \affiliation{\Parisuniversite}
\author{T.~Safford} \affiliation{\Michiganstate}
\author{N.~Sahu} \affiliation{\IndHyderabad}
\author{P.~Sala} \affiliation{\INFNMilano}\affiliation{\CERN}
\author{G.~Salukvadze} \affiliation{\CERN}
\author{N.~Samios} \affiliation{\Brookhaven}
\author{M.~C.~Sanchez} \affiliation{\IowaState}
\author{D.~A.~Sanders} \affiliation{\Mississippi}
\author{D.~Sankey} \affiliation{\Rutherford}
\author{S.~Santana} \affiliation{\PuertoRico}
\author{M.~Santos-Maldonado} \affiliation{\PuertoRico}
\author{N.~Saoulidou} \affiliation{\Athens}
\author{P.~Sapienza} \affiliation{\INFNSud}
\author{C.~Sarasty} \affiliation{\Cincinnati}
\author{I.~Sarcevic} \affiliation{\Arizona}
\author{G.~Savage} \affiliation{\Fermi}
\author{V.~Savinov} \affiliation{\Pitt}
\author{A.~Scaramelli} \affiliation{\INFNPavia}
\author{A.~Scarff} \affiliation{\Sheffield}
\author{A.~Scarpelli} \affiliation{\Brookhaven}
\author{H.~Schellman} \affiliation{\OregonState}\affiliation{\Fermi}
\author{P.~Schlabach} \affiliation{\Fermi}
\author{D.~Schmitz} \affiliation{\Chicago}
\author{K.~Scholberg} \affiliation{\Duke}
\author{A.~Schukraft} \affiliation{\Fermi}
\author{E.~Segreto} \affiliation{\Campinas}
\author{E.~Seltskaya} \affiliation{\CERN}
\author{J.~Sensenig} \affiliation{\Penn}
\author{I.~Seong} \affiliation{\CalIrvine}
\author{A.~Sergi} \affiliation{\Birmingham}
\author{F.~Sergiampietri} \affiliation{\StonyBrook}
\author{D.~Sgalaberna} \affiliation{\ETH}
\author{M.~H.~Shaevitz} \affiliation{\Columbia}
\author{S.~Shafaq} \affiliation{\Jawaharlal}
\author{M.~Shamma} \affiliation{\CalRiverside}
\author{H.~R.~Sharma} \affiliation{\Jammu}
\author{R.~Sharma} \affiliation{\Brookhaven}
\author{T.~Shaw} \affiliation{\Fermi}
\author{C.~Shepherd-Themistocleous} \affiliation{\Rutherford}
\author{S.~Shin} \affiliation{\Jeonbuk}
\author{D.~Shooltz} \affiliation{\Michiganstate}
\author{R.~Shrock} \affiliation{\StonyBrook}
\author{L.~Simard} \affiliation{\Lal}
\author{N.~Simos} \affiliation{\Brookhaven}
\author{J.~Sinclair} \affiliation{\Bern}
\author{G.~Sinev} \affiliation{\Duke}
\author{J.~Singh} \affiliation{\Lucknow}
\author{J.~Singh} \affiliation{\Lucknow}
\author{V.~Singh} \affiliation{\CUSB}\affiliation{\Banaras}
\author{R.~Sipos} \affiliation{\CERN}
\author{F.~W.~Sippach} \affiliation{\Columbia}
\author{G.~Sirri} \affiliation{\INFNBologna}
\author{A.~Sitraka} \affiliation{\SouthDakotaSchool}
\author{K.~Siyeon} \affiliation{\ChungAng}
\author{D.~Smargianaki} \affiliation{\StonyBrook}
\author{A.~Smith} \affiliation{\Duke}
\author{A.~Smith} \affiliation{\Cambridge}
\author{E.~Smith} \affiliation{\Indiana}
\author{P.~Smith} \affiliation{\Indiana}
\author{J.~Smolik} \affiliation{\CzechTechnical}
\author{M.~Smy} \affiliation{\CalIrvine}
\author{P.~Snopok} \affiliation{\Illinoisinstitute}
\author{M.~Soares Nunes} \affiliation{\Campinas}
\author{H.~Sobel} \affiliation{\CalIrvine}
\author{M.~Soderberg} \affiliation{\Syracuse}
\author{C.~J.~Solano Salinas} \affiliation{\Ingenieria}
\author{S.~S\"{o}ldner-Rembold} \affiliation{\Manchester}
\author{N.~Solomey} \affiliation{\Wichita}
\author{V.~Solovov} \affiliation{\LIP}
\author{W.~E.~Sondheim} \affiliation{\LosAlmos}
\author{M.~Sorel} \affiliation{\IFIC}
\author{J.~Soto-Oton} \affiliation{\CIEMAT}
\author{A.~Sousa} \affiliation{\Cincinnati}
\author{K.~Soustruznik} \affiliation{\Charles}
\author{F.~Spagliardi} \affiliation{\Oxford}
\author{M.~Spanu} \affiliation{\Brookhaven}
\author{J.~Spitz} \affiliation{\Michigan}
\author{N.~J.~C.~Spooner} \affiliation{\Sheffield}
\author{K.~Spurgeon} \affiliation{\Syracuse}
\author{R.~Staley} \affiliation{\Birmingham}
\author{M.~Stancari} \affiliation{\Fermi}
\author{L.~Stanco} \affiliation{\INFNPadova}
\author{D.~Stefan} \affiliation{\CERN}
\author{H.~M.~Steiner} \affiliation{\LawrenceBerkeley}
\author{J.~Stewart} \affiliation{\Brookhaven}
\author{B.~Stillwell} \affiliation{\Chicago}
\author{J.~Stock} \affiliation{\SouthDakotaSchool}
\author{F.~Stocker} \affiliation{\CERN}
\author{T.~Stokes} \affiliation{\Louisanastate}
\author{M.~Strait} \affiliation{\Minntwin}
\author{T.~Strauss} \affiliation{\Fermi}
\author{S.~Striganov} \affiliation{\Fermi}
\author{A.~Stuart} \affiliation{\Colima}
\author{R.~Sulej} \affiliation{\NCNR}\affiliation{\Fermi}
\author{D.~Summers} \affiliation{\Mississippi}
\author{A.~Surdo} \affiliation{\INFNLecce}
\author{V.~Susic} \affiliation{\Basel}
\author{L.~Suter} \affiliation{\Fermi}
\author{C.~M.~Sutera} \affiliation{\CataniaUniversitadi}\affiliation{\INFNCatania}
\author{R.~Svoboda} \affiliation{\CalDavis}
\author{B.~Szczerbinska} \affiliation{\TexasAM}
\author{A.~M.~Szelc} \affiliation{\Manchester}
\author{R.~Talaga} \affiliation{\Argonne}
\author{H. A.~Tanaka} \affiliation{\SLAC}
\author{B.~Tapia Oregui} \affiliation{\Texasaustin}
\author{A.~Tapper} \affiliation{\Imperial}
\author{S.~Tariq} \affiliation{\Fermi}
\author{E.~Tatar} \affiliation{\Idaho}
\author{R.~Tayloe} \affiliation{\Indiana}
\author{A.~M.~Teklu} \affiliation{\StonyBrook}
\author{M.~Tenti} \affiliation{\INFNBologna}
\author{K.~Terao} \affiliation{\SLAC}
\author{C.~A.~Ternes} \affiliation{\IFIC}
\author{F.~Terranova} \affiliation{\INFNMilanBicocca}\affiliation{\MilanoBicocca}
\author{G.~Testera} \affiliation{\INFNGenova}
\author{A.~Thea} \affiliation{\Rutherford}
\author{J.~L.~Thompson} \affiliation{\Sheffield}
\author{C.~Thorn} \affiliation{\Brookhaven}
\author{S.~C.~Timm} \affiliation{\Fermi}
\author{A.~Tonazzo} \affiliation{\Parisuniversite}
\author{M.~Torti} \affiliation{\INFNMilanBicocca}\affiliation{\MilanoBicocca}
\author{M.~Tortola} \affiliation{\IFIC}
\author{F.~Tortorici} \affiliation{\CataniaUniversitadi}\affiliation{\INFNCatania}
\author{D.~Totani} \affiliation{\Fermi}
\author{M.~Toups} \affiliation{\Fermi}
\author{C.~Touramanis} \affiliation{\Liverpool}
\author{J.~Trevor} \affiliation{\Caltech}
\author{W.~H.~Trzaska} \affiliation{\Jyvaskyla}
\author{Y.~T.~Tsai} \affiliation{\SLAC}
\author{Z.~Tsamalaidze} \affiliation{\Georgian}
\author{K.~V.~Tsang} \affiliation{\SLAC}
\author{N.~Tsverava} \affiliation{\Georgian}
\author{S.~Tufanli} \affiliation{\CERN}
\author{C.~Tull} \affiliation{\LawrenceBerkeley}
\author{E.~Tyley} \affiliation{\Sheffield}
\author{M.~Tzanov} \affiliation{\Louisanastate}
\author{M.~A.~Uchida} \affiliation{\Cambridge}
\author{J.~Urheim} \affiliation{\Indiana}
\author{T.~Usher} \affiliation{\SLAC}
\author{M.~R.~Vagins} \affiliation{\Kavli}
\author{P.~Vahle} \affiliation{\WilliamMary}
\author{G.~A.~Valdiviesso} \affiliation{\FederaldeAlfenas}
\author{E.~Valencia} \affiliation{\WilliamMary}
\author{Z.~Vallari} \affiliation{\Caltech}
\author{J.~W.~F.~Valle} \affiliation{\IFIC}
\author{S.~Vallecorsa} \affiliation{\CERN}
\author{R.~Van Berg} \affiliation{\Penn}
\author{R.~G.~Van de Water} \affiliation{\LosAlmos}
\author{D.~Vanegas Forero} \affiliation{\Campinas}
\author{F.~Varanini} \affiliation{\INFNPadova}
\author{D.~Vargas} \affiliation{\IFAE}
\author{G.~Varner} \affiliation{\Hawaii}
\author{J.~Vasel} \affiliation{\Indiana}
\author{G.~Vasseur} \affiliation{\CEASaclay}
\author{K.~Vaziri} \affiliation{\Fermi}
\author{S.~Ventura} \affiliation{\INFNPadova}
\author{A.~Verdugo} \affiliation{\CIEMAT}
\author{S.~Vergani} \affiliation{\Cambridge}
\author{M.~A.~Vermeulen} \affiliation{\Nikhef}
\author{M.~Verzocchi} \affiliation{\Fermi}
\author{H.~Vieira de Souza} \affiliation{\Campinas}
\author{C.~Vignoli} \affiliation{\GranSassoLab}
\author{C.~Vilela} \affiliation{\StonyBrook}
\author{B.~Viren} \affiliation{\Brookhaven}
\author{T.~Vrba} \affiliation{\CzechTechnical}
\author{T.~Wachala} \affiliation{\Niewodniczanski}
\author{A.~V.~Waldron} \affiliation{\Imperial}
\author{M.~Wallbank} \affiliation{\Cincinnati}
\author{H.~Wang} \affiliation{\CalLosangeles}
\author{J.~Wang} \affiliation{\CalDavis}
\author{Y.~Wang} \affiliation{\CalLosangeles}
\author{Y.~Wang} \affiliation{\StonyBrook}
\author{K.~Warburton} \affiliation{\IowaState}
\author{D.~Warner} \affiliation{\ColoradoState}
\author{M.~Wascko} \affiliation{\Imperial}
\author{D.~Waters} \affiliation{\UniversityCollegeLondon}
\author{A.~Watson} \affiliation{\Birmingham}
\author{P.~Weatherly} \affiliation{\Drexel}
\author{A.~Weber} \affiliation{\Rutherford}\affiliation{\Oxford}
\author{M.~Weber} \affiliation{\Bern}
\author{H.~Wei} \affiliation{\Brookhaven}
\author{A.~Weinstein} \affiliation{\IowaState}
\author{D.~Wenman} \affiliation{\Wisconsin}
\author{M.~Wetstein} \affiliation{\IowaState}
\author{M.~R.~While} \affiliation{\SouthDakotaSchool}
\author{A.~White} \affiliation{\TexasArlington}
\author{L.~H.~Whitehead} \affiliation{\Cambridge}
\author{D.~Whittington} \affiliation{\Syracuse}
\author{M.~J.~Wilking} \affiliation{\StonyBrook}
\author{C.~Wilkinson} \affiliation{\Bern}
\author{Z.~Williams} \affiliation{\TexasArlington}
\author{F.~Wilson} \affiliation{\Rutherford}
\author{R.~J.~Wilson} \affiliation{\ColoradoState}
\author{J.~Wolcott} \affiliation{\Tufts}
\author{T.~Wongjirad} \affiliation{\Tufts}
\author{K.~Wood} \affiliation{\StonyBrook}
\author{L.~Wood} \affiliation{\PacificNorthwest}
\author{E.~Worcester} \affiliation{\Brookhaven}
\author{M.~Worcester} \affiliation{\Brookhaven}
\author{C.~Wret} \affiliation{\Rochester}
\author{W.~Wu} \affiliation{\Fermi}
\author{W.~Wu} \affiliation{\CalIrvine}
\author{Y.~Xiao} \affiliation{\CalIrvine}
\author{G.~Yang} \affiliation{\StonyBrook}
\author{T.~Yang} \affiliation{\Fermi}
\author{N.~Yershov} \affiliation{\INR}
\author{K.~Yonehara} \affiliation{\Fermi}
\author{T.~Young} \affiliation{\Northdakota}
\author{B.~Yu} \affiliation{\Brookhaven}
\author{H.~W.~Yu} \affiliation{\Brookhaven}
\author{H.~Z.~Yu} \affiliation{\SunYatSen}
\author{J.~Yu} \affiliation{\TexasArlington}
\author{Z.~Y.~Yu} \affiliation{\IHEP}
\author{R.~Zaki} \affiliation{\York}
\author{J.~Zalesak} \affiliation{\CzechAcademyofSciences}
\author{L.~Zambelli} \affiliation{\DannecyleVieux}
\author{B.~Zamorano} \affiliation{\Granada}
\author{A.~Zani} \affiliation{\CERN}\affiliation{\INFNMilano}
\author{L.~Zazueta} \affiliation{\WilliamMary}
\author{G.~P.~Zeller} \affiliation{\Fermi}
\author{J.~Zennamo} \affiliation{\Fermi}
\author{K.~Zeug} \affiliation{\Wisconsin}
\author{C.~Zhang} \affiliation{\Brookhaven}
\author{M.~Zhao} \affiliation{\Brookhaven}
\author{E.~Zhivun} \affiliation{\Brookhaven}
\author{G.~Zhu} \affiliation{\Ohiostate}
\author{E.~D.~Zimmerman} \affiliation{\ColoradoBoulder}
\author{M.~Zito} \affiliation{\CEASaclay}
\author{S.~Zucchelli} \affiliation{\INFNBologna}\affiliation{\BolognaUniversity}
\author{J.~Zuklin} \affiliation{\CzechAcademyofSciences}
\author{V.~Zutshi} \affiliation{\Northernillinois}
\author{R.~Zwaska} \affiliation{\Fermi}
%973 authors
%----------------------------------------------------
\collaboration{The DUNE Collaboration}
%\noaffiliation


==> trigger.tex <==
\section{Event trigger}
\label{sec:trigger}

In order to perform event selection a hardware trigger system was developed. The system is composed by an interface board with an FPGA and a CPU to establish an interface between the different detection inputs (photon detectors, beam instrumentation, cosmic-ray taggers - CRT) and the DAQ through the timing system.

The trigger electronics received 32 individual CRT pixel inputs (a pixel being a unit of two overlapping panels), 24 photon detector inputs and individual beam instrumentation signals.

%suggestion for rework on the text above:
A hardware triggering system was designed in order to perform event selection in ProtoDUNE-SP.
The core element of this system is the Central Trigger Board (CTB) which is a custom printed circuit board (PCB) in charge of processing the status of the auxiliary detectors to aid in making prompt readout decisions.
The readout decisions are ultimately made by the timing system which communicates with the CTB through various commands.
The CTB itself, hosts a Microzed, which is a commercial PCB with an onboard System-On-a-Chip (SoC).
The SoC contains both Programmable Logic (PL) and a Processing System (PS) and serves as an interface between the auxiliary detectors (PDS, beam instrumentation, and CRT) and the DAQ through the timing system.
The CTB has 32 individual CRT pixel inputs (a pixel being a unit of two overlapping panels), 24 optical inputs for the SSPs, and seven inputs for beam instrumentation signals, all of which, are translated into digital pulses and forwarded to the PL for further processing.

%TODO: Maybe add a picture of the CTB? I don't see pictures of other modules such as the SSPs, so maybe not..

%suggested additional paragraph to explain the firmware (at least minimally):
The CTB triggering firmware operating in the PL is organized into a two-level hierarchy of Low-Level and High-Level Triggers (LLTs and HLTs) which are configurable at run-time by the DAQ system. 
LLTs are defined for inputs from a single subsystem while HLTs can be defined using the various LLTs and can therefore span any or a combination of the subsystems.
Several trigger conditions can be set up; each one is uniquely identified by a bitmask and is embedded into a trigger word issued to the DAQ.
Additionally, multiple trigger conditions can be met during a single event; to distinguish between these, the CTB timestamps all LLTs and HLTs generated with the 50 MHz system clock. This (64-bit) timestamp is also included in the trigger word along with the bitmask.

Several trigger conditions could be set up, each one being individually identified to the DAQ. Using bitmasks, the configured trigger conditions could either require a particular signal to be present, or to not be present. For example, one could create a condition of the form "detector \textit{a} has a signal outside of beam gate", which would require the bit for detector \textit{a} to be asserted \textbf{and} the \textit{beam gate} bit to be deasserted. 
Only when all the required conditions were met, a trigger command was passed to the timing system, which was responsible for validating the issued trigger (in case a sufficient elapsed time since the last trigger had passed) and then propagating it both to the DAQ software and the individual readout systems.

Regardless of a trigger being validated by the timing system, all trigger conditions were timestamped with a 50 MHz clock in sync with the rest of the detector, and a data word was sent to the DAQ to be stored along with the remainder of the detector data. 

%suggestion for rework of the original text above:
At the high level, trigger conditions can be configured to require coincidences or anti-coincidences between the various LLTs.
For example, one could create a condition of the form "auxiliary detector \textit{a} has a signal outside of the beam gate", which would require the bit for detector \textit{a} to be asserted \textbf{and} the \textit{beam gate} bit to be deasserted.
Only when all the required conditions for an HLT are met, is a trigger command passed to the timing system. 
The timing system is then responsible for validating or vetoing\footnote{In case a trigger has already been issued by the timing system.} the issued trigger. 
If accepted, the timing system forwards the readout decision to both the DAQ software and the individual readout systems (i.e. PDS, CRT, and TPC).
However, for accountability\footnote{If beam pile-up occurs, the timing system would veto any additional beam triggers if it has issued one in the last 10~ms. However, the CTB would still report multiple beam triggers.}, the CTB sends a data word directly to the DAQ to be stored regardless of whether or not the trigger is validated by the timing system.

Using this setup, several different types of trigger were put in place that can be divided into two classes: \textit{beam on} triggers, that relied mostly in the beam instrumentation inputs and required the conditions to be met during a beam spill; and \textit{beam off} triggers, which required the conditions to be met outside the beam spill. 

%suggested rework for the original text above:
% My understanding from what Tingjun suggested was that we avoided making the description too technical, and focus on the physics capabilities. The whole concept of LLT and HLT is one of those things that I would argue will confuse more than help.
% If we are to put this, then we *must* add a diagram of the internals of the CTB. Personally I think it is overkill.
All HLTs can be classified as \textit{beam on} or \textit{beam off} triggers.
The former relies mostly on the beam instrumentation inputs and requires the conditions to be met during a beam spill while the latter requires that the conditions be met outside the beam spill.
The most common examples of beam on triggers include those aimed at tagging electron, proton and kaon events.
By requiring different signal combinations from the beam instrumentation inputs, one can identify specific particles for a relevant energy range, as shown in table \ref{tab:PID}.

The most common examples of the former class of triggers included triggers aimed to tag electron, proton and kaon events. By requiring different signal combinations from the beam instrumentation inputs, one could identify specific particles for a relevant energy range, as shown in table \ref{tab:PID}. In fact, all the conditions identified in table \ref{tab:PID} were set up as individual triggers. 

The most common examples of the latter class of triggers were cosmic-ray triggers. Several of these kinds of triggers were in place to select events with specific topologies, requiring CRT panels from specific regions to register hits in coincidence with panels from another region. For example, by requiring at least one upstream CRT panel to have a hit in coincidence with a downstream CRT panel, throughgoing horizontal muons are selected. Another trigger set up following this procedure was for plane crossing muons, which could be achieved by requiring coincidence hits on CRT counters on opposing drift volumes and sides of the cryostat. 

%suggested rework for the original text above:
The most common examples of beam off triggers are those arising from cosmic-ray activity. Several of this class of triggers are in place to select events with specific topologies, requiring CRT pixels from specific regions to register hits in coincidence with pixels from another region. 
For example, by requiring that at least one upstream CRT pixel is hit in coincidence with a downstream CRT pixel, one can select through-going muon candidates. 
Another trigger is set up for cathode-crossing muon candidates, which is achieved by requiring coincidence hits on CRT pixels on opposing drift volumes and sides of the cryostat.

Besides the logic specific triggers, a minimal-bias (or random trigger) was also put in place to lead readout of the detector in the absence of any particular trigger condition. This random trigger was set up to fire at 1~Hz.

%suggested rework for the original text above:
Aside from the logic-specific triggers, a minimum-bias (i.e. random) trigger is in place to lead to the readout of the detector in the absence of any particular trigger condition.
The capability to issue random triggers is built into the timing system. %as well as the CTB, but we mainly used the ones from the timing system. The ones from the CTB were mainly useful for debugging
Random triggers can be toggled during a run by the run control and their frequency is tunable.


